I Have an Attention Bridge to Sell You: Generalization Capabilities of Modular Translation Architectures

Modularity is a paradigm of machine translation with the potential of bringing forth models that are large at training time and small during inference. Within this field of study, modular approaches, and in particular attention bridges, have been argued to improve the generalization capabilities of models by fostering language-independent representations. In the present paper, we study whether modularity affects translation quality; as well as how well modular architectures generalize across different evaluation scenarios. For a given computational budget, we find non-modular architectures to be always comparable or preferable to all modular designs we study.

==> figs/lin-layers.tex <==
\begin{tikzpicture}[
% GLOBAL CFG
%font=\sf \scriptsize,
>=LaTeX,
% Styles
cell/.style={% For the main box
    rectangle,
    rounded corners=2.5mm,
    draw,
    line width = 1.5pt,
    },
operator/.style={%For operators like +  and  x
    circle,
    draw,
    inner sep=-0.5pt,
    line width = 1pt,
    minimum height =.2cm,
    },
function/.style={%For functions
    ellipse,
    draw,
    line width = 1pt,
    inner sep=1pt
    },
ct/.style={% For external inputs and outputs
    circle,
    draw,
    line width = 1pt,
    minimum width=1cm,
    inner sep=.5pt,
    },
gt/.style={% For internal inputs
    rectangle,
    draw,
    minimum width=4mm,
    minimum height=3mm,
    inner sep=1.5pt,
    line width=1pt,
    },
mylabel/.style={% something new that I have learned
    font=\scriptsize\sffamily
    },
ArrowC1/.style={% Arrows with rounded corners
    rounded corners=.3cm,
    line width=1pt,
    },
ArrowC2/.style={% Arrows with big rounded corners
    rounded corners=.75cm,
    line width=1pt,
    },
]

\node [cell, minimum height =5cm, minimum width=5cm] (lin) at (0, -0.5){} ;

\node [ct] (wq) at (-1.75,-2) {$\mathbf{W}_Q$};
\node [ct] (wk) at (0,-2) {$\mathbf{W}_K$};
\node [] (wv) at (1.75,-2) {};

\node [gt] (frelu) at (0,-0.875) {$\phi(~\cdots~)^\top$};
\node [gt] (fmatmul1) at (-0.875,0) {$\mathrm{matmul}$};
\node [gt] (fsoftmax) at (-0.875,0.875) {$\mathrm{softmax}(~\cdots~)$};
\node [gt] (fmatmul2) at (0,1.625) {$\mathrm{matmul}$};

\node[ct] (ipt) at (0, -3.75) {$\mathbf{X}$};
%\node[ct] (opt) at (0, 3) {$\mathbf{Y}$};
\draw [->, ArrowC1] (ipt.north) -- (wk.south);
\draw [ArrowC1] (ipt.east) -| (wv.center);
\draw [ArrowC1] (wk.north) -- (frelu.south);
\draw [ArrowC1] (wq.north) |- (fmatmul1.west);
\draw [ArrowC1] (frelu.north) |- (fmatmul1.east);
\draw [ArrowC1] (fmatmul1.north) -- (fsoftmax.south);
\draw [ArrowC1] (fsoftmax.north) |- (fmatmul2.west);
\draw [->, ArrowC1] (wv.center) |- (fmatmul2.east);

\draw [decorate,decoration={brace,amplitude=3mm, raise=.5mm},line width=1pt] (lin.north east) -- (lin.south east);
\node[right=0.5cm of lin,text width=3.25cm]{\larger\larger \cref{eq:lin}, applied for all $\mathcal{L}$ variants ($\mathcal{L}$, $\mathcal{L}^\mathrm{f}$, $\mathcal{L}^\mathrm{f}_\mathrm{p}$ \& $\mathcal{L}_\mathrm{p}$)};


\node [cell, minimum height=3.5cm, minimum width=5cm] (ff) at (0, 4){} ;
\node [ct] (win) at (0,3.125) {$\mathbf{W}_I$};
\node [gt] (fpsi) at (0, 4.125) {$\phi(~\cdots~)$};
\node [ct] (wout) at (0,5.125) {$\mathbf{W}_O$};

\draw [->, ArrowC1] (fmatmul2.north) -- (win.south);
\draw [ArrowC1] (win.north) -- (fpsi.south);
\draw [ArrowC1] (fpsi.north) -- (wout.south);

\draw [decorate,decoration={brace,amplitude=3mm, raise=.5mm},line width=1pt] (ff.north east) -- (ff.south east);
\node[right=0.5cm of ff,text width=3cm]{\larger\larger\cref{eq:ff}, applied  for $\mathcal{L}^\mathrm{f}$ and $\mathcal{L}^\mathrm{f}_\mathrm{p}$};

\node [cell, minimum height=2.125cm, minimum width=5cm] (pe) at (0, 7){} ;
\node [gt] (fadd) at (0, 7.625) {$\mathrm{add}$};
\node [ct] (wpe) at (-1.75, 6.625) {$\mathbf{P}$};

\draw [->, ArrowC1] (wout.north) -- (fadd.south);
\draw [ArrowC1] (wpe.north) |- (fadd.west);

\draw [decorate,decoration={brace,amplitude=3mm, raise=.5mm},line width=1pt] (pe.north east) -- (pe.south east);
\node[right=0.5cm of pe,text width=3cm]{\larger\larger\cref{eq:pe}, applied  for $\mathcal{L}_\mathrm{p}^\mathrm{f}$ and $\mathcal{L}_\mathrm{p}$};

\node[ct] (opt) at (0, 9) {$\mathbf{\hat{Y}}$};
\draw [->, ArrowC1] (fadd.north) -- (opt.south);

\end{tikzpicture}
